Volumetric Occupancy Detection: A Comparative Analysis of Mapping Algorithms

Despite the growing interest in innovative functionalities for collaborative robotics, volumetric detection remains indispensable for ensuring basic security. However, there is a lack of widely used volumetric detection frameworks specifically tailored to this domain, and existing evaluation metrics primarily focus on time and memory efficiency. To bridge this gap, the authors present a detailed comparison using a simulation environment, ground truth extraction, and automated evaluation metrics calculation. This enables the evaluation of state-of-the-art volumetric mapping algorithms, including OctoMap, SkiMap, and Voxblox, providing valuable insights and comparisons through the impact of qualitative and quantitative analyses. The study not only compares different frameworks but also explores various parameters within each framework, offering additional insights into their performance.

==> Makefile <==
.PHONY: all build preview print ebook cleanall clean

# Vars
SRC     := ${PWD}
OUT     := ${PWD}/build
SCRIPTS := ${PWD}/scripts

# Commands
LATEXMK := latexmk
LATEXMK_FLAGS := -pdf
#LATEXMK_FLAGS += -silent
LATEXMK_FLAGS += -view=pdf
LATEXMK_FLAGS += -auxdir=${OUT}
LATEXMK_FLAGS += -outdir=${OUT}
LATEXMK_FLAGS += -pdflatex="pdflatex -file-line-error --shell-escape %O %S"
# LATEXMK_FLAGS += -e '$$makeindex=q/sh -c "cd `dirname "%D"`" ; makeindex %O -o "`basename "%D"`" "`basename "%S"`";/'

all: build

build:
	cd ${OUT} ; ${LATEXMK} ${LATEXMK_FLAGS} -cd ${SRC}/matter.tex

preview: build
	(${LATEXMK} ${LATEXMK_FLAGS} -pvc -cd ${SRC}/matter.tex)

print: build
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dNOPAUSE -dQUIET -dBATCH -sOutputFile=${OUT}/thesis-print.pdf ${OUT}/matter.pdf
	${SCRIPTS}/simplify-colors.sh ${OUT}/thesis-print.pdf

ebook: build
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/ebook -dNOPAUSE -dQUIET -dBATCH -sOutputFile=${OUT}/thesis-ebook.pdf ${OUT}/matter.pdf

clean:
	@find ${OUT} -type f ! -name '*.pdf' ! -name '.*' -exec rm "{}" \;

cleanall:
	@find ${OUT} -type f ! -name '.*' -exec rm "{}" \;

lint:
ifeq ($(strip $(texfile)),)
	+@for f in `ls -v chapters/*.tex`; do  \
		echo "* $$f";  \
		make --no-print-directory lint texfile="$$f";  \
	done
else
	@lacheck "$(texfile)"
	@chktex -q --verbosity=3 "$(texfile)"
	$(eval txtfile := $(shell echo "$(OUT)/`basename "$(texfile)" .tex`.txt"))
	@pandoc -s "$(texfile)" -o "$(txtfile)"
	@proselint "$(txtfile)" || true
endif

